Cross-corpus Readability Compatibility Assessment for English Texts

Text readability assessment has gained significant attention from researchers in various domains. However, the lack of exploration into corpus compatibility poses a challenge as different research groups utilize different corpora. In this study, we propose a novel evaluation framework, Cross-corpus text Readability Compatibility Assessment (CRCA), to address this issue. The framework encompasses three key components: (1) Corpus: CEFR, CLEC, CLOTH, NES, OSP, and RACE. Linguistic features, GloVe word vector representations, and their fusion features were extracted. (2) Classification models: Machine learning methods (XGBoost, SVM) and deep learning methods (BiLSTM, Attention-BiLSTM) were employed. (3) Compatibility metrics: RJSD, RRNSS, and NDCG metrics. Our findings revealed: (1) Validated corpus compatibility, with OSP standing out as significantly different from other datasets. (2) An adaptation effect among corpora, feature representations, and classification methods. (3) Consistent outcomes across the three metrics, validating the robustness of the compatibility assessment framework. The outcomes of this study offer valuable insights into corpus selection, feature representation, and classification methods, and it can also serve as a beginning effort for cross-corpus transfer learning.

==> CRCA_appendices.tex <==

\appendices
\section{}
\label{appendix:index score}

% Table 3 Readability formula scores of datasets
\renewcommand{\arraystretch}{1.2} % 设置表格中每一行的行高
\begin{table}[htp]
\caption{Readability formula scores of datasets}
\centering
\footnotesize
\resizebox{8.5cm}{!}{
\begin{tabular}{llllllllll}
\toprule[1.5pt]
Class        & ARI    & FKGL   & GFI    & SMOG  & CLI   & LIX    & RIX   \\
\midrule
\multicolumn{8}{c}{CEFR}                                                 \\
\hline
A1           & 2.57   & 2.83   & 7.01   & 7.25  & 4.24  & 21.79  & 1.19  \\
A2           & 3.81   & 3.55   & 7.03   & 7.14  & 5.31  & 24.98  & 1.62  \\
B1           & 8.10   & 7.06   & 10.68  & 9.87  & 8.51  & 36.40  & 3.31  \\
B2           & 7.89   & 7.04   & 10.75  & 9.77  & 8.26  & 36.09  & 3.26  \\
C1           & 10.56  & 9.24   & 13.14  & 11.66 & 10.63 & 43.55  & 4.67  \\
C2           & 11.26  & 10.00  & 14.21  & 12.27 & 10.16 & 44.23  & 4.94  \\
\hline
\multicolumn{8}{c}{CLEC}                                                 \\
\hline
ST2          & 51.25  & 40.63  & 44.63  & 20.62 & 12.07 & 122.40 & 22.08 \\
ST3          & 65.69  & 52.04  & 56.60  & 26.80 & 14.34 & 151.91 & 32.51 \\
ST4          & 60.05  & 47.46  & 52.25  & 24.19 & 14.13 & 140.05 & 27.44 \\
ST5          & 90.88  & 72.00  & 76.35  & 29.57 & 15.40 & 203.17 & 49.48 \\
ST6          & 151.10 & 119.72 & 125.63 & 43.99 & 16.06 & 324.29 & 88.71 \\
\hline
\multicolumn{8}{c}{CLOTH}                                                \\
\hline
middle       & 3.87   & 3.08   & 7.58   & 7.30  & 4.46  & 25.86  & 1.77  \\
high         & 7.26   & 5.74   & 10.66  & 9.05  & 5.71  & 33.48  & 2.79  \\
\hline
\multicolumn{8}{c}{NES}                                                  \\
\hline
2nd grade    & 2.85   & 3.09   & 5.64   & 6.75  & 5.82  & 23.23  & 1.20  \\
3rd grade    & 4.45   & 4.43   & 6.90   & 7.62  & 7.49  & 27.50  & 1.69  \\
4th grade    & 5.44   & 5.27   & 7.87   & 8.26  & 8.08  & 30.08  & 2.11  \\
5th grade    & 6.93   & 6.60   & 9.18   & 9.16  & 9.21  & 34.10  & 2.73  \\
6th grade    & 8.20   & 7.74   & 10.38  & 9.92  & 9.69  & 37.19  & 3.34  \\
7th grade    & 9.46   & 8.89   & 11.47  & 10.68 & 10.57 & 40.53  & 3.97  \\
8th grade    & 10.55  & 9.70   & 12.39  & 11.18 & 10.63 & 42.72  & 4.50  \\
9th grade    & 11.65  & 10.75  & 13.38  & 11.89 & 11.39 & 45.61  & 5.12  \\
10th grade   & 11.66  & 10.69  & 13.50  & 11.91 & 11.11 & 45.51  & 5.13  \\
12th grade   & 13.09  & 11.87  & 14.69  & 12.60 & 11.37 & 48.54  & 5.93  \\
\hline
\multicolumn{8}{c}{OSP}                                                  \\
\hline
beginner     & 8.56   & 7.55   & 11.06  & 10.29 & 9.24  & 36.96  & 3.42  \\
intermediate & 10.60  & 9.41   & 13.03  & 11.65 & 10.29 & 42.17  & 4.47  \\
advanced     & 12.14  & 10.67  & 14.39  & 12.51 & 10.87 & 45.99  & 5.33  \\
\hline
\multicolumn{8}{c}{RACE}                                                 \\
\hline
middle       & 5.09   & 5.17   & 8.13   & 7.85  & 5.92  & 28.26  & 2.17  \\
high         & 10.37  & 9.57   & 12.54  & 10.88 & 9.27  & 41.33  & 4.50 \\
\bottomrule[1.5pt]
\end{tabular}
}

\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{}
\label{appendix:Distribution}

\begin{figure}[htp]
    \centering
    \includegraphics[width=8.5cm]{Dis_ARI.pdf}
    \caption{Distribution ARI Grade per Text by Reading Labels}
\end{figure}

\begin{figure}[htp]
    \centering    
    \includegraphics[width=8.5cm]{Dis_FleschKincaidGradeLevel.pdf}
    \caption{Distribution FKGL Grade per Text by Reading Labels}
\end{figure}

\begin{figure}[htp]
    \centering
    \includegraphics[width=8.5cm]{Dis_GunningFogIndex.pdf}
    \caption{Distribution GFI Grade per Text by Reading Labels}
\end{figure}

\begin{figure}[htp]
    \centering
    \includegraphics[width=8.5cm]{Dis_SMOGIndex.pdf}
    \caption{Distribution SMOG Grade per Text by Reading Labels}
\end{figure}

\begin{figure}[htp]
    \centering
    \includegraphics[width=8.5cm]{Dis_ColemanLiauIndex.pdf}
    \caption{Distribution CLI Grade per Text by Reading Labels}
\end{figure}

\begin{figure}[htp]
    \centering    
    \includegraphics[width=8.5cm]{Dis_LIX.pdf}
    \caption{Distribution LIX Grade per Text by Reading Labels}
\end{figure}

\begin{figure}[htp]
    \centering
    \includegraphics[width=8.5cm]{Dis_RIX.pdf}
    \caption{Distribution RIX Grade per Text by Reading Labels}
\end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\newpage

\section{}
\label{appendix:Feature}

% Table 2: Feature Information
\begin{table}[h]
\centering
\caption{Feature Information}
\renewcommand{\arraystretch}{1.2}
\label{tab:Information}
\resizebox{9cm}{!}{
\begin{tabular}{ccl}
\toprule[1.5pt]
Count & Code & Description \\
\hline
\multicolumn{3}{c}{Lexical Features}  \\
\hline
0     & ALPW & average letters per word                                                   \\
1     & ASPW & average syllables per word                                                  \\
2     & CWP  & percentage of complex words                                                \\
3     &  DWP  & percentage of difficult words                                                 \\
4     & LWP  & percentage of long words                                                     \\
\hline
\multicolumn{3}{c}{Syntactic Features}                                                      \\
\hline
5     & ANPS & average length of noun phrases                                               \\
6     & APPS & average length of prepositional phrases                                      \\
7     & APT  & average length of parse tree                                                 \\
8     & AVPS & average length of verb phrases                                               \\
9     & AWPS & average number of words per sentence                                         \\
10    & LSP  & percentage of long sentences                                                 \\
11    & NPS  & average number of noun phrases per sentence                                  \\
12    & PPS  & average number of prepositional phrases per sentence                         \\
13    & SPS  & average number of subordinate clauses per sentence                           \\
14    & SQS  & average number of special subordinate clause per sentence \\
15    & VPS  & average number of verb phrases per sentence                                  \\
\hline
\multicolumn{3}{c}{Grammatical Features}                                                    \\
\hline
16    & CoP  & percentage of conjunctions                                                   \\
17    & CP   & percentage of commas\\
18    & NP   & percentage of nouns                                                          \\
19    & PNP  & percentage of proper nouns                                                   \\
20    & PP   & percentage of pronouns                                                       \\         \bottomrule[1.5pt]                                             
\end{tabular}
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \pagebreak
\section{}
\label{appendix:Model Performance}

\begin{table}[htp]
\renewcommand{\arraystretch}{1}
% \setlength{\tabcolsep}{1.5pt}
\caption{Model Performance}
% \caption{Model Performance}
% \label{model performance}\\
% 表格“首页”显示内容
\resizebox{8.5cm}{!}{
\begin{tabular}{lccccc}
\toprule
\quad   & Method     & Accuracy & Precision & Recall & F1 \\
\midrule
% \endfirsthead

% % “后续页面”表头显示内容
% \multicolumn{6}{r}{Continued}\\
% \toprule
% \quad & Method     & Accuracy & Precision & Recall & F1 \\
% %\midrule
% \endhead

% % 表格“尾页前”，表格最后显示内容
% %\bottomrule
% \multicolumn{6}{c}{Continued on next page}\\
% \endfoot

% 表格“尾页”，表格最后显示内容3*4
% \bottomrule
% \endlastfoot
\multicolumn{6}{c}{CEFR} \\
\hline
\multirow{2}{*}{Feature} 
& XGBoost & 0.416    & 0.207     & 0.290  & 0.222 \\
& SVM        & 0.415    & 0.291     & 0.363  & 0.278 \\
\hline
\multirow{4}{*}{GloVe}         
& XGBoost    & 0.431    & 0.283     & 0.325  & 0.287 \\
& SVM        & 0.547    & 0.552     & 0.512  & 0.525 \\
& BiLSTM     & 0.309    & 0.232     & 0.205  & 0.154 \\
& Att-BiLSTM & 0.300    & 0.085     & 0.141  & 0.102 \\
\hline
\multirow{4}{*}{Fusion Feature} 
& XGBoost    & 0.387    & 0.492     & 0.371  & 0.385 \\
& SVM        & 0.518    & 0.475     & 0.545  & 0.503 \\
& BiLSTM     & 0.373    & 0.896     & 0.167  & 0.091 \\
& Att-BiLSTM & 0.327    & 0.598     & 0.155  & 0.104 \\
\hline
\multicolumn{6}{c}{CLEC}\\
\toprule
\multirow{2}{*}{Feature}      
& XGBoost    & 0.416    & 0.207     & 0.290  & 0.222 \\
& SVM        & 0.415    & 0.291     & 0.363  & 0.278 \\
\hline
\multirow{4}{*}{GloVe}        
& XGBoost    & 0.431    & 0.309     & 0.376  & 0.292 \\
& SVM        & 0.528    & 0.229     & 0.428  & 0.326 \\
& BiLSTM     & 0.394    & 0.497     & 0.363  & 0.328 \\
& Att-BiLSTM & 0.411    & 0.243     & 0.362  & 0.260 \\
\hline
\multirow{4}{*}{Fusion Feature} 
& XGBoost    & 0.401    & 0.287     & 0.351  & 0.267 \\
& SVM        & 0.528    & 0.298     & 0.455  & 0.351 \\
& BiLSTM     & 0.478    & 0.464     & 0.421  & 0.378 \\
& Att-BiLSTM & 0.406    & 0.703     & 0.362  & 0.260 \\
\hline
\multicolumn{6}{c}{CLOTH}\\
\toprule
\multirow{2}{*}{Feature}       
& XGBoost    & 0.732    & 0.726     & 0.727  & 0.727 \\
& SVM        & 0.750    & 0.501     & 0.489  & 0.492 \\
\hline
\multirow{4}{*}{GloVe}         
& XGBoost    & 0.746    & 0.740     & 0.739  & 0.739 \\
& SVM        & 0.773    & 0.768     & 0.769  & 0.769 \\
& BiLSTM     & 0.593    & 0.711     & 0.514  & 0.400 \\
& Att-BiLSTM & 0.751    & 0.829     & 0.705  & 0.705 \\
\hline
\multirow{4}{*}{Fusion Feature} 
& XGBoost    & 0.783    & 0.779     & 0.776  & 0.777 \\
& SVM        & 0.818    & 0.813     & 0.815  & 0.814 \\
& BiLSTM     & 0.834    & 0.836     & 0.822  & 0.827 \\
& Att-BiLSTM & 0.831    & 0.831     & 0.819  & 0.823 \\
\hline
\multicolumn{6}{c}{NES}\\
\toprule
\multirow{2}{*}{Feature}       
& XGBoost    & 0.272    & 0.170     & 0.239  & 0.179 \\
& SVM        & 0.275    & 0.176     & 0.241  & 0.181 \\
\hline
\multirow{4}{*}{GloVe}         
& XGBoost    & 0.157    & 0.100     & 0.127  & 0.084 \\
& SVM        & 0.452    & 0.366     & 0.353  & 0.343 \\
& BiLSTM     & 0.271    & 0.091     & 0.195  & 0.105 \\
& Att-BiLSTM & 0.195    & 0.157     & 0.124  & 0.068 \\
\hline
\multirow{4}{*}{Fusion Feature} 
& XGBoost    & 0.274    & 0.191     & 0.263  & 0.198 \\
& SVM        & 0.286    & 0.198     & 0.277  & 0.208 \\
& BiLSTM     & 0.513    & 0.690     & 0.359  & 0.281 \\
& Att-BiLSTM & 0.516    & 0.665     & 0.373  & 0.329 \\
\hline
\multicolumn{6}{c}{OSP}\\
\toprule
\multirow{2}{*}{Feature}       
& XGBoost    & 0.605    & 0.641     & 0.605  & 0.616 \\
& SVM        & 0.561    & 0.474     & 0.421  & 0.431 \\
\hline
\multirow{4}{*}{GloVe}         
& XGBoost    & 0.605    & 0.719     & 0.605  & 0.613 \\
& SVM        & 0.623    & 0.612     & 0.623  & 0.617 \\
& BiLSTM     & 0.484    & 0.467     & 0.474  & 0.446 \\
& Att-BiLSTM & 0.264    & 0.500     & 0.269  & 0.223 \\
\hline
\multirow{4}{*}{Fusion Feature} 
& XGBoost    & 0.614    & 0.663     & 0.614  & 0.623 \\
& SVM        & 0.728    & 0.733     & 0.728  & 0.729 \\
& BiLSTM     & 0.363    & 0.669     & 0.364  & 0.238 \\
& Att-BiLSTM & 0.429    & 0.754     & 0.411  & 0.308 \\
\hline
\multicolumn{6}{c}{RACE}\\
\toprule
\multirow{2}{*}{Feature}       
& XGBoost    & 0.837    & 0.527     & 0.511  & 0.518 \\
& SVM        & 0.775    & 0.856     & 0.563  & 0.548 \\
\hline
\multirow{4}{*}{GloVe}         
& XGBoost    & 0.819    & 0.819     & 0.815  & 0.817 \\
& SVM        & 0.837    & 0.836     & 0.835  & 0.836 \\
& BiLSTM     & 0.751    & 0.715     & 0.537  & 0.506 \\
& Att-BiLSTM & 0.850    & 0.816     & 0.779  & 0.795 \\
\hline
\multirow{4}{*}{Fusion Feature} 
& XGBoost    & 0.850    & 0.823     & 0.759  & 0.782 \\
& SVM        & 0.846    & 0.845     & 0.844  & 0.845 \\
& BiLSTM     & 0.822    & 0.778     & 0.737  & 0.752 \\
& Att-BiLSTM & 0.850    & 0.816     & 0.778  & 0.794\\
\hline
\end{tabular}
}
\end{table}
